Breaking the Sample Complexity Barrier to Regret-Optimal Model-Free Reinforcement Learning

Achieving sample efficiency in online episodic reinforcement learning (RL) requires optimally balancing exploration and exploitation. When it comes to a finite-horizon episodic Markov decision process with $S$ states, $A$ actions and horizon length $H$, substantial progress has been achieved towards characterizing the minimax-optimal regret, which scales on the order of $\sqrt{H^2SAT}$ (modulo log factors) with $T$ the total number of samples. While several competing solution paradigms have been proposed to minimize regret, they are either memory-inefficient, or fall short of optimality unless the sample size exceeds an enormous threshold (e.g., $S^6A^4 \,\mathrm{poly}(H)$ for existing model-free methods). To overcome such a large sample size barrier to efficient RL, we design a novel model-free algorithm, with space complexity $O(SAH)$, that achieves near-optimal regret as soon as the sample size exceeds the order of $SA\,\mathrm{poly}(H)$. In terms of this sample size requirement (also referred to the initial burn-in cost), our method improves -- by at least a factor of $S^5A^3$ -- upon any prior memory-efficient algorithm that is asymptotically regret-optimal. Leveraging the recently introduced variance reduction strategy (also called {\em reference-advantage decomposition}), the proposed algorithm employs an {\em early-settled} reference update rule, with the aid of two Q-learning sequences with upper and lower confidence bounds. The design principle of our early-settled variance reduction method might be of independent interest to other RL settings that involve intricate exploration-exploitation trade-offs.

==> offline-main-results.tex <==
\section{Offline RL algorithms and theoretical guarantees}
\label{sec:algorithm-theory-lcbq}


In the current paper, we present two model-free algorithms --- namely, \LCBQ and {\LCBQR} --- for offline RL, along with their respective theoretical guarantees. The first algorithm can be viewed as a pessimistic variant of the classical Q-learning algorithm, 
while the second one further leverages the idea of variance reduction to boost the sample efficiency. In this section, we begin by introducing \LCBQ.





\subsection{\LCBQ: a natural pessimistic variant of Q-learning}


Before proceeding, we find it convenient to first review the classical Q-learning algorithm \citep{watkins1989learning,watkins1992q}, which can be regarded as a stochastic approximation scheme to solve the Bellman optimality equation \eqref{eq:bellman_optimality}. 
Upon receiving a sample transition $(s_h,a_h,r_h,s_{h+1})$ at time step $h$, 
Q-learning updates the corresponding entry in the Q-estimate as follows
\begin{align}    \label{eq:classical-Q-update}
    Q_h(s_h,a_h) ~\leftarrow~ & (1-\eta )Q_h(s_h,a_h)  + \eta \Big \{ r_h(s_h,a_h) + 
  V_{h+1}(s_{h+1}) \Big \} ,
\end{align}
where $Q_h$ (resp.~$V_h$) indicates the running estimate of $Q_h^{\star}$ (resp.~$V_h^{\star}$), and $0<\eta<1$ is the learning rate. 
In comparison to model-based algorithms that require estimating the probability transition kernel based on all the samples, Q-learning, as a popular kind of model-free algorithms, is simpler and enjoys more flexibility without explicitly constructing the model of the environment.
The wide applicability of Q-learning motivates one to adapt it to accommodate offline RL. 


% The advantage of Q-learning over model-based algorithms lies in its memory and computational efficiency, which does not require explicit construction of the transition kernel. Therefore, it is of great interest to explore if Q-learning can be adapted for offline RL in a provably-efficient manner.


Inspired by recent advances in incorporating the pessimism principle for offline RL \citep{rashidinejad2021bridging,jin2021pessimism}, 
we study a pessimistic variant of Q-learning called \LCBQ, which modifies the Q-learning update rule as follows
\begin{align}
    \label{equ:lcb-q-update}
    Q_h(s_h, a_h) \leftarrow & (1-\eta_n )Q_h(s_h, a_h) + \eta_n \Big\{ r_h(s_h,a_h) +  V_{h+1}(s_{h+1})  - b_n \Big\}, 
\end{align}
%
where $\eta_n$ is the learning rate depending on the number of times $n$ that the state-action pair $(s_h,a_h)$ has been visited at step $h$, and the penalty term $b_n>0$ (cf.~line~\ref{line:2} of Algorithm~\ref{algo:lcb-index}) reflects the uncertainty of the corresponding Q-estimate and implements pessimism in the face of uncertainty. 
The entire algorithm, which is a {\em single-pass} algorithm that only requires reading the offline dataset once, 
is summarized in Algorithm~\ref{algo:lcb-index}. 
 
 

 
 

\begin{algorithm}[h]
 \textbf{Parameters:} some constant $\cb>0$, target success probability $1-\delta \in(0,1)$, and $\iota = \log\big(\frac{SAT}{\delta}\big)$. \\
\textbf{Initialize}  $Q_h(s, a) \leftarrow 0$, $N_h(s, a)\leftarrow 0$, and $V_h(s) \leftarrow 0$ for all $(s,a,h)\in \cS\times \cA\times[H+1]$; $\widehat{\pi}$ s.t. $\widehat{\pi}_h(s) = 1$ for all $(h,s)\in [H]\times\cS$.  \\
\For{Episode $ k = 1$ \KwTo $K$}{
	Sample a new trajectory $\{s_h, a_h, r_h\}_{h=1}^H$ from $\mathcal{D}_{\mu}$. {\small\color{own_blue}\tcp{sampling from batch dataset}} 
   {\small\color{own_blue}\tcp{update the policy} }  \normalsize
%	Compute $\widehat{\pi}$ s.t.~$\widehat{\pi}_h(s) = \arg\max_a Q_{h}(s, a)$ for any $(s,h)\in \cS\times[H]$. \label{line:lcb-policy-update}\\
  \For{Step $ h = 1$ \KwTo $H$}{
    
    
         $N_h(s_h, a_h) \leftarrow N_h(s_h, a_h) + 1$. {\small\color{own_blue}\tcp{update the counter} }
   
         $n \leftarrow N_h(s_h, a_h)$; 
        $\eta_n \leftarrow \frac{H + 1}{H + n}$.  
        {\small\color{own_blue}\tcp{update the learning rate}}      
        $b_n \leftarrow \cb \sqrt{\frac{H^3\iota^2}{n}}$.  \label{line:2-nok}  {\small\color{own_blue}\tcp{update the bonus term}}
        {\small\color{own_blue}\tcp{run the Q-learning update with LCB} }  \normalsize
  $Q_h(s_h, a_h) \leftarrow Q_h(s_h, a_h) + \eta_n\Big\{ r_h(s_h, a_h) + V_{h+1}(s_{h+1})-Q_h(s_h, a_h) - b_n \Big\} 
  $. \label{line:lcb-9-nok} \\
          
     {\small\color{own_blue}\tcp{update the value estimates}} \normalsize
      
    $V_{h}(s_h) \leftarrow \max\Big\{ V_{h}(s_h), \,  \max_a Q_{h}(s_h, a)  \Big\}$. \label{line:lcb_v_update}\\
    \label{line:lcb-10}
    If $V_{h}(s_h) = \max_a Q_{h}(s_h, a)$: update $\widehat{\pi}_h(s) \leftarrow \arg\max_a Q_{h}(s, a)$.
 %   {\small\color{blue}\tcc{update for other state-action pair except $s_h^k, a_h^k$}} \normalsize
 %   $\left(N_h^{k+1}(s,a) ,Q_h^{k+1}(s,a)\right) \leftarrow \left(N_h^k(s,a),Q_h^{k}(s,a)\right)$ for all $(s,a) \neq (s_h^k, a_h^k)$.\\
%    $V_h^{k+1}(s) \leftarrow V_h^{k}(s)$ for all $s \neq s_h^k$. 
 }
 }
 \textbf{Output:} the policy $\widehat{\pi}$.
\caption{\LCBQ for offline RL}
\label{algo:lcb-index}
\end{algorithm}






\subsection{Theoretical guarantees for \LCBQ{}}
 
The proposed {\LCBQ{}} algorithm manages to achieve an appealing sample complexity as formalized by the following theorem. 
%
\begin{theorem}\label{thm:lcb}
  Consider any $\delta \in (0,1)$.
  Suppose that the behavior policy $\mu$ satisfies Assumption~\ref{assumption} with single-policy concentrability coefficient $C^{\star}\geq 1$. Let $\cb>0$ be some sufficiently large constant, and take $\iota \coloneqq \log\big(\frac{SAT}{\delta}\big)$. Assume that $T>SC^\star \iota$, then the policy $\widehat{\pi}$ returned by Algorithm~\ref{algo:lcb-index} satisfies
%
\begin{align}\label{equ:lcb-result}
    V_1^\star(\rho) - V_1^{\widehat{\pi}}(\rho) 
  %&\leq \max_{1\leq h\leq H} \sum_{s\in \cS} d_h^{\pi^\star}(s) \big(V_h^{\star}(s) - V_h^{\widehat{\pi}}(s) \big) \nonumber\\
  &\leq c_\mathrm{a} \sqrt{\frac{H^6 SC^\star \iota^3}{T}} 
  %+  \frac{H^3 SC^\star \iota}{T} 
\end{align}
%
with probability at least $1-\delta$, where $c_\mathrm{a}>0$ is some universal constant. 
\end{theorem}
%\lxs{Should we remove $\frac{H^3 SC^\star \iota}{T}$ since it will always been dominated by $\sqrt{\frac{H^6 SC^\star \iota}{T}}$? 
%$$ \begin{cases} \frac{H^3 SC^\star \iota}{T} \leq \sqrt{\frac{H^6 SC^\star \iota}{T}} & \text{ if } T\geq SC^\star \iota\\ V_1^\star(\rho) - V_1^{\widehat{\pi}}(\rho) \leq H \leq H^3 \leq \sqrt{\frac{H^6 SC^\star \iota}{T}} & \text{ if } T < SC^\star \iota \end{cases}$$ }
%\yuting{then we need to assume $T>SC^\star \iota$}

 As asserted by Theorem~\ref{thm:lcb}, the {\LCBQ{}} algorithm is guaranteed to find an $\varepsilon$-optimal policy with high probability, 
 as long as the total sample size $T=KH$ exceeds
 %
 \begin{equation}
  \widetilde{O}\left( \frac{H^6 S C^\star}{\varepsilon^2} \right),
   \label{eq:lcb-sample-complexity}
\end{equation} 
where $\widetilde{O}(\cdot)$ hides logarithmic dependencies. When the behavior policy is close to the optimal policy, the single-policy concentrability coefficient $C^{\star}$ is closer to 1; if this is the case, then our bound indicates that the sample complexity does not depend on the size $A$ of the action space, which can be a huge saving when the action space is enormous.


\paragraph{Comparison with model-based pessimistic approaches.} 

A model-based approach --- called Value Iteration with Lower Confidence Bounds  (\VILCB) ---
has been recently proposed for offline RL \citep{rashidinejad2021bridging,xie2021policy}. 
In the finite-horizon case, \VILCB{} incorporates an additional LCB penalty into the classical value iteration algorithm, and updates {\em all} the entries in the Q-estimate simultaneously as follows
%
\begin{align}
    Q_h(s,a) ~\leftarrow~ r_h(s,a) + \widehat{P}_{h,s,a}V_{h+1} - b_h(s,a), \label{equ:VI-UCB}
\end{align}
%
with the aim of tuning down the confidence on those state-action pairs that have only been visited infrequently. 
Here, $\widehat{P}_{h,s,a}$ represents the empirical estimation of the transition kernel $P_{h,s,a}$, 
and $b_h(s,a) >0$ is chosen to capture the uncertainty level of $(\widehat{P}_{h,s,a} -P_{h,s,a})V_{h+1}$. 
Working backward, the algorithm estimates the Q-value $Q_h$ recursively over the time steps $h = H, H-1, \cdots, 1$.  In comparison with \VILCB, our sample complexity bound for  {\LCBQ{}} matches the bound developed for \VILCB{} by \citet{xie2021policy}, while enjoying enhanced flexibility without the need of specifying the transition kernel of the environment (as model estimation might potentially incur a higher memory burden).  

